On a linear stability issue of split form schemes for compressible flows

Split form schemes for Euler and Navier-Stokes equations are useful for computation of turbulent flows due to their better robustness. This is because they satisfy additional conservation properties of the governing equations like kinetic energy preservation leading to a reduction in aliasing errors at high orders. Recently, linear stability issues have been pointed out for these schemes for a density wave problem and we investigate this behaviour for some standard split forms. By deriving linearized equations of split form schemes, we show that most existing schemes do not satisfy a perturbation energy equation that holds at the continuous level. A simple modification to the energy flux of some existing schemes is shown to yield a scheme that is consistent with the energy perturbation equation. Numerical tests are given using a discontinuous Galerkin method to demonstrate these results.

==> postp/tables.tex <==
\begin{document}

\begin{table}
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
$N$ & $4 \times 4$ & $6 \times 6$ & $8 \times 8$ & $10 \times 10$ \\
\hline
3 &              &          &  & \\
\hline
4 &              &          &  & \\
\hline
5 &              &          &  & \\
\hline
\end{tabular}
\end{center}
\caption{Density wave test in 2-D}
\end{table}

\begin{table}[!h]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
  & Av   & Ducros & KG   & mKEP \\
  \hline
3 & 0.51 & 0.51   & 0.13 & 0.51 \\
\hline
4 & 0.49 & 0.49   & 0.07 & 0.49 \\
\hline
5 & 10   & 10     & 0.08 & 10  \\
\hline
\end{tabular}
\end{center}
\caption{Time to blow-up for density wave test for $4 \times 4$ mesh. Tests were run until $T=10$.}
\end{table}


\begin{table}[!h]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
  & Av   & Ducros & KG   & mKEP \\
  \hline
3 & 1.60 & 1.60   & 0.14 & 1.60 \\
\hline
4 & 10 & 10   & 0.17 & 10 \\
\hline
5 & 10   & 10     & 0.10 & 10  \\
\hline
\end{tabular}
\end{center}
\caption{Time to blow-up for density wave test for $6 \times 6$ mesh. Tests were run until $T=10$.}
\end{table}

\begin{table}[!h]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
  & Av   & Ducros & KG   & mKEP \\
  \hline
3 & 10 & 10   & 0.09 & 10 \\
\hline
4 & 10 & 10   & 0.08 & 10 \\
\hline
5 & 10   & 10     & 0.08 & 10  \\
\hline
\end{tabular}
\end{center}
\caption{Time to blow-up for density wave test for $8 \times 8$ mesh. Tests were run until $T=10$.}
\end{table}


\begin{table}[!h]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
  & Av   & Ducros & KG   & mKEP \\
  \hline
3 & 10 & 10   & 0.15 & 10 \\
\hline
4 & 10 & 10   & 0.09 & 10 \\
\hline
5 & 10   & 10     & 0.14 & 10  \\
\hline
\end{tabular}
\end{center}
\caption{Time to blow-up for density wave test for $10 \times 10$ mesh. Tests were run until $T=100$. $\Delta x_{eff} = 1/20$}
\end{table}

\begin{table}[!h]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
  & Av   & Ducros & KG   & mKEP \\
  \hline
1E-3 & 0.80 & 7.48   & 0.08 & 5.79 \\
\hline
1E-4 & 40.22 & 40.22   & 0.08 & 49.17 \\
\hline
1E-5 & 100   & 100     & 0.08 & 100  \\
\hline
\end{tabular}
\end{center}
\caption{Time to blow-up for density wave test with perturbation for $4 \times 4$ mesh, N=5. Tests were run until $T=100$. $\Delta x_{eff} = 1/20$}
\end{table}

\begin{table}[!h]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
  & Av   & Ducros & KG   & mKEP \\
  \hline
1E-3 & 3.90 & 3.90   & 0.07 & 2.47 \\
\hline
1E-4 & 20.83 & 20.83   & 0.10 & 20.84 \\
\hline
1E-5 & 100   & 100     & 0.10 & 100  \\
\hline
\end{tabular}
\end{center}
\caption{Time to blow-up for density wave test with perturbation for $8 \times 8$ mesh, N=3. Tests were run until $T=100$. $\Delta x_{eff} = 1/24$}
\end{table}


\begin{table}[!h]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
  & Av   & Ducros & KG   & mKEP \\
  \hline
1E-3 & 5.50 & 7.27   & 0.15 & 5.47 \\
\hline
1E-4 & 36.13 & 36.13   & 0.09 & 36.15 \\
\hline
1E-5 & 100   & 100     & 0.09 & 100  \\
\hline
\end{tabular}
\end{center}
\caption{Time to blow-up for density wave test with perturbation for $10 \times 10$ mesh, N=3. Tests were run until $T=100$. $\Delta x_{eff} = 1/30$}
\end{table}

\begin{table}[!h]
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
  & Av   & Ducros & KG   & mKEP \\
  \hline
1E-3 & 2.50 & 9.13   & 0.08 & 9.88 \\
\hline
1E-4 & 77.47 & 84.56   & 0.09 & 100 \\
\hline
1E-5 & 100   & 100     & 0.09 & 100  \\
\hline
\end{tabular}
\end{center}
\caption{Time to blow-up for density wave test with perturbation for $8 \times 8$ mesh, N=4. Tests were run until $T=100$. $\Delta x_{eff} = 1/32$}
\end{table}

\end{document}
